Distributed Freeze Tag: a Sustainable Solution to Discover and Wake-up a Robot Swarm

The Freeze Tag Problem consists in waking up a swarm of robots starting with one initially awake robot. Whereas there is a wide literature of the centralized setting, where the location of the robots is known in advance, we focus in the distributed version where the location of the robots $\P$ are unknown, and where awake robots only detect other robots up to distance~$1$. Assuming that moving at distance $\delta$ takes a time $\delta$, we show that waking up of the whole swarm takes $O(\rho+\ell^2\log( \rho/\ell))$, where $\rho$ stands for the largest distance from the initial robot to any point of $\P$, and the $\ell$ is the connectivity threshold of $\P$. Moreover, the result is complemented by a matching lower bound in both parameters $\rho$ and $\ell$. We also provide other distributed algorithms, complemented with lower bounds, whenever each robot has a bounded amount of energy.

==> fig/separator/fig_separator.tex <==
\begin{figure}[h!]
    \captionsetup[subfigure]{position=b}
    \centering
    
    %\label{fig:Mould}
    \subcaptionbox{\textsf{Initialization} \label{fig:initialization-sep}}{\includegraphics[width=.3\linewidth]{fig/separator/0INIT.pdf}}
    \subcaptionbox{\dfsampling from $s$ to get a sample of size $4\ell$.\label{fig:DFS-sep}}{\includegraphics[width=.3\linewidth]{fig/separator/1DFS.pdf}}
    \subcaptionbox{\textsf{Exploration} of $4$ separators by teams of $\ell$ robots. \label{fig:exploration-sep}}{\includegraphics[width=.3\linewidth]{fig/separator/2EXPLO.pdf}}
    \caption{$\bullet$ Sleeping robots $\circ$ awake robots  \tikzbullet{blue-source}{black} sleeping source  \tikzbullet{blue-source}{white} awake source}
\end{figure}


\begin{comment}
\begin{figure}[htb!]
    \centering
    \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\textwidth]{fig/separator/0INIT.pdf}
        %\def\svgwidth{0.8\textwidth}
        %\input{fig/separator/pdftex/0INIT.pdf_tex}
        %\caption{\label{fig:initialization-sep}}
    \caption{\textsf{Initialization} \label{fig:initialization-sep}}
    %\caption{\textsf{Initialization} and \textsf{Recruitment} during Round 0. \dfsampling from $s$ to get a sample of size $4\ell$.\label{fig:DFS-sep}}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{fig/separator/1DFS.pdf}
        \caption{\dfsampling from $s$ to get a sample of size $4\ell$.\label{fig:DFS-sep}}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{fig/separator/2EXPLO.pdf}
        \caption{\textsf{Exploration} of $4$ separators by teams of $\ell$ robots. \label{fig:exploration-sep}}
    \end{subfigure}%
    %\caption{\textsf{Initialization} and \textsf{Recruitment} during Round 0.}
    \caption{$\bullet$ Sleeping robots $\circ$ awake robots  \tikzbullet{blue-source}{black} sleeping source  \tikzbullet{blue-source}{white} awake source \Taissir{TODO - pourquoi ça fait une erreur de compilation ???? + ajuster alignement des sous-images}}
\end{figure}
\end{comment}

==> old-algos.tex <==
% Contient (dans l'ordre):
% Recruitment (pseudo-code)
% DFS (pseudo-code)
% DiscoverSolo (pseudo-code + preuve)
% discovermany (pseudo-code)
% Separator (pseudo-code)


%%%%% Recruitement
\begin{algorithm}[H]
\caption{\textsc{Recruitment} - pseudo-code}
\KwIn{$\team_i, \X_i$}
$\team(\squarereg[i]) \gets \X_i$\;
\ForEach{$s \in \textsc{MonotonicPath}(\X_i)$}{
    \lIf{$|\team(\squarereg[i])| \geq L$}{\stop}%
    $\stack \gets \{s\}$\;
    \While{$|\team(\squarereg[i])| \geq L$ \KwAnd \xspace \stack\xspace  \KwNot null}{
        $\nxt \gets \stack.\pop$\;
        $\move(\nxt)$\;
        $\wakeup(\nxt)$\;
        $\team(\squarereg[i]) \gets \team(\squarereg[i]) \cup \{\nxt\}$\;
        $\stack.\push(\textsc{Discover}(B_{s}(L), \team_i) \backslash \team(\squarereg[i]))$\;
    }
}
\end{algorithm}
%%%%% Fin Recruitement
%%%%% DFS
\subsubsection{Naive DFS}
\Gabriel{On va probablement vouloir définir des fonctions plus que des algorithmes, au sens où on voudra appeler dans une fonction une autre fonction, avec des arguments particuliers}

\begin{algorithm}[H]
\caption{\textsc{Naive DFS} - code for $u_i$}
\textsc{Update}(k, ctr, stack)\; % à son réveil, le robot "apprend" l'information partagée par les robots réveillés
stack.\textsc{Push}(\textsc{Discovery}($p_i$, L, ctr))\;
\While{ctr $<$ k \KwAnd stack \KwNot null}{
    ctr $\leftarrow$ ctr$+ 1$\;
    nxt$\leftarrow$ stack.\textsc{Pop}()\;
    \textsc{MoveTo}(nxt)\;
    \textsc{WakeUp}(nxt)\; %départ de DFS 
    \textsc{Share}(ctr, k, stack)\; % en réalité, seul nxt apprend
}
\end{algorithm}
At each iteration $i\in [1, k]$, a team of $i + 1$ robots $(u_0, u_1, u_2, ..., u_i)$ explores a surface of size $2 \pi L^2$ in order to wake up the next robot $u_{i+1}$. The exploration is distributed between the robots so each of them explore a surface of $\frac{2\pi L^2}{i}$ and consequently the exploration time decrease at each step, unless no new robot is discovered. In this case if $ctr < k$ the team backtracks i.e moves to the next position stored in $stack$ and start again the exploration. Backtracking can occurs at most $k$ times. Let $T_{DFS}(k)$ be the overall time complexity of the \textsc{DFS} wake up for $k$ robots.
\begin{align*}
    T_{DFS}(k) \leq kL + \sum^{k}_{i=0} \frac{2\pi L^2}{i} = O(L^2\log k + kL)
\end{align*}
%%%% Fin DFS

%%%% Discover Solo
\begin{algorithm}
    \caption{\textsc{Function DiscoverSolo, which discovers a rectangle with given corners, executed by $u$}}
    \Input{$(x_0, y_0)$ and $(x_f, y_f)$ such that $(x_0, y_0) \preceq (x_f, y_f)$ and $(x_0, y_0)$ is the initial position of $u$ in the beginning of the execution}
    \KwVar{x, y, \forcex, \forcey, \orientation, \discovered}
    \Output{\discovered, set of position of sleeping robots in $\rect((x_0, y_0),(x_f, y_f))$}
    \Guarantee{the position of $u$ in the end of the execution is $(x_f, y_f)$}
    $\discovered := \emptyset$;\\
    $x := x_0 + \sqrt 3/2$;\\
    $y := y_0 + 1/2$;\\
    $\orientation := 1$;\\
    $\forcex := \KwTrue$;\\
    % $\move((x_0, y_0), (x,y))$;\\
    \While{$x \leq x_f - \sqrt 3/2$ \KwOr $\forcex$}{
        $\forcex := \KwFalse$;\\
        $\forcey := \KwTrue$;\\
        \While{$y_0 + 1/2 \leq y \leq y_f - 1/2$ \KwOr $\forcey$}{
            $\forcey := \KwFalse$;\\
            $\move((x,y))$;\\
            $\discovered := \discovered \cup \snap()$;\\
            $y := y+\orientation$;\\
        }
        $y:= y-\orientation$;\\
        $\orientation := - \orientation$;\\
        $x := x + \sqrt 3$;\\
    }
    $\move((x_f, y_f))$;\label{algosolo:final_move}\\
\end{algorithm}

\begin{lemma}
    At the end of the execution of $DiscoverSolo(p_0, p_f)$, $\discovered$ contains all the robots that are still asleep in the end of the execution, and whose initial position is in $\rect(p_0,p_f)$.
\end{lemma}
\begin{proof}
    Note first that a snapshot taken at position $(x_i + \sqrt3/2, y_i+1/2)$ detects all the robots in $\rect((x_i, y_i), (x_i+\sqrt 3, y_i+1))$.
    Note first that along the execution, the tuple $\snap()$ is executed at positions $(x,y)$, for all values $(x,y)$ in \dots
\end{proof}
\begin{lemma}
    The duration of $DiscoverSolo(p_0, p_f)$ is less than $\frac{XY}{\sqrt 3} + X + Y + 2$, where $X = x_f-x_0$ and $Y = y_f - y_0$.
\end{lemma}
\begin{proof}
    First note that the duration of the move of line~\ref{algosolo:final_move} is at most $Y$.
    The number of  cycles of the inner loop is $\max(1, \lfloor Y \rfloor)$.
    The duration of the first cycle is $1$ or $\sqrt 3$, and the duration of the others is $1$.
    The number of cycles of the outer loop is $\max (1, \lfloor \frac{X}{\sqrt 3} \rfloor)$.
    \begin{itemize}
        \item
            If $Y\geq 1$ and $\lfloor \frac X{\sqrt 3} \rfloor \geq 1$, then the duration of the execution is:
        
                    $\lfloor \frac{X}{\sqrt 3} \rfloor \times (\sqrt 3 + Y-1) \leq \frac{XY}{\sqrt 3} + X$.
        \item
            If $Y\geq 1$ and $\lfloor \frac X{\sqrt 3} \rfloor < 1$, then the duration of the execution is:
            
            $\sqrt 3 + Y - 1 \leq Y + 1$.
        \item
            If $Y < 1$ and $\lfloor \frac X{\sqrt 3} \rfloor \geq 1$, then the duration of the execution is:
            
            $\lfloor \frac{X}{\sqrt 3} \rfloor \times \sqrt 3 \leq X$.
        \item
            If $Y < 1$ and $\lfloor \frac X{\sqrt 3} \rfloor < 1$, then the duration of the execution is: $1$.
    \end{itemize}
\end{proof}
%%%% Fin DiscoverSolo

%%%% Discover Many
\begin{algorithm}
    \caption{\textsc{Function DiscoverMany, which collectively discovers a piece of a rectangle with given corners, executed by $u$}}
    \Input{$(x_0, y_0)$ and $(x_f, y_f)$ such that $(x_0, y_0) \preceq (x_f, y_f)$ and $(x_0, y_0)$ is the initial position of $u$ in the beginning of the execution}
    \KwVar{\msg, \teamsize, \index, \step, \discovered}
    \Output{\discovered, set of position of sleeping robots in $\rect((x_0, y_0),(x_f, y_f))$}
    \Guarantee{the position of $u$ in the end of the execution is $(x_f, y_f)$}

    $\msg := \share()$;\\
    $\teamsize := |\msg|$;\\
    $\index := |\{\msg \mid \msg.I < I_u\}|$;\tcc*{j'ai mis id faute de mieux} %\\
    $\step := \frac{x_f - x_0}{\teamsize}$;\\
    $\move((x_0+\step*\index,y_0))$;\\
    $\discovered := DiscoverSolo((x_0+\step*\index,y_0), (x_0+(\step+1)*\index,y_f))$;\\
    $\move((x_f, y_f))$;\\
    $\wait(value ?)$;\tcc*{ICI gérer une synchro} %\\
    $\msg := \share()$;\\
    $\discovered := \cup_{m\in \msg} m.\discovered$;\\
\end{algorithm}

%%%% Fin Discover Many

%%%% Separator
\begin{algorithm}
\caption{\textsc{Separator} Global pseudo code}
\KwIn{$\team, \squarereg$}
\KwPreCond{$|\team | \geq L$ and the whole team $\team$ is co-localized at the center of \squarereg}

\If{$R \leq L^{\frac{3}{2}}$}{
     $X \gets \textsc{Discover}(\squarereg, \team)$\tcc*{Exploration of \squarereg with $L$ robots}
     $\wut \gets \diskwakeup(\squarereg, \team)$\tcc*{Centralized computation of a wake up tree in \squarereg}
     $\propagatewut(\wut, \team)$\;
     $\stop$\;
}
$\team_1,\team_2,\team_3,\team_4 \gets \textsc{split}(\team)$\tcc*{Divide \team into four teams of $\frac{L}{4}$ robots}
$\squarereg[1],\squarereg[2],\squarereg[3],\squarereg[4] \gets \textsc{split}(\squarereg)$\tcc*{Divide \squarereg into four sub squares with side length $\frac{R}{2}$}
\ForParallel{$i \in [1, 4]$}{
    $X_i \gets \textsc{Discover}(\squarereg[i]^{L-\square}, \team_i)$\tcc*{Discover position in a $L$-wide border in $\squarereg[i]$ \Taissir{Détailler la mise à jour des connaissances antérieures}}
    $\visited \gets []$\;
    $seeds \gets X_i$\;
    \While(\tcc*{\Taissir{Recrutement de robots : soit (1) détailler dans une procédure séaprée, probablement. Ou (2) écrire moins technique}}){$|X_i| \leq L$}{
        $s \gets seeds.\pop()$\;
        $\textsc{Recruit}(s, \team_i)$\tcc*{This should update the state of visited and seeds.}
        \tcc*{\Taissir{j'ai abandonné avant de finir cette boucle..}}
    }
} %end for in parallel
Awake robots gather in the center of $\squarereg$ and share known positions\;
\ForParallel{$i \in [1, 4]$}{
    $\team_i \gets$ tous les robots natifs de $\squarereg[i]$\;
    $\team_i \move$ au centre de $\squarereg[i]$\;
    \eIf(\tcc{This ensure the pre-condition on teamsize}){$|\team_i| \leq L$}{%
        \stop\tcc*{Thm: no sleeping robots left in $\squarereg[i]$}
    }{
        $\textsc{Separator}(\team_i, \squarereg[i])$\;
    }
}
\end{algorithm}
%%%% Fin Separator








% https://arxiv.org/pdf/2107.04885 https://www.researchgate.net/publication/271629959_Gathering_on_rings_under_the_Look-Compute-Move_model https://epubs.siam.org/doi/10.1137/S009753979732428X https://arxiv.org/pdf/2102.13062 https://people.cis.ksu.edu/~rhowell/asymptotic.pdf -> ref intéressantes ? -- Gabriel

Old Model :


\paragraph{Computational hypotheses.}

\begin{enumerate}[label=(\roman*)]

    \item Robots are uniquely identified, typically by their initial position $p_i$.

    \item Robots are considered as $0$-dimensional points: several robots can gather at the same position.

    \item Communication between robots is only possible between robots located a
    t the same point.

    \item Robots share common absolute space coordinates \label{comput-hyp:space}

    \item Robots are given a clock which is synchronized on all awake robots \label{comput-hyp:time}

    \item Precision on time and space coordinates is infinite

    \item Robots have no restriction on the memory usage
    % \item Robots have a primitive {\sf detect} which detects and stores the position of any sleeping robot which belongs to $B_{{\sf pos}(\rob_i, t)}(1)$ \Gabriel{Pas sûr en fait, on va plutôt essayer de coder ça avec des snapshot de Boule 1 discrets qui couvrent intégralement la surface à couvrir, avec une redondance nécessaire, mais bornée.}
    
    \item Robots can use several \emph{actions}, with associated \emph{trace}
        \begin{itemize}
            % \item $\wait(t)$ of duration $t$ and trace the empty word,
            % \item $\move(p_i, p_f)$ of duration $|p_ip_f|$ and trace $(p_i, p_f)$,
            % \item $\snap(p_i)$ of duration $0$ and trace $(p_i, p_i)$,
            % \item $\wakeup(r)$ of duration $0$ and trace $(p_r, p_r)$,
            % \item $\share()$ of duration $0$ and trace the empty word.
            \item $\wait(t)$ of trace the empty word,
            \item $\move(p)$ of trace $m_p$,
            \item $\snap()$ of trace the empty word,
            \item $\wakeup(p, args)$ of trace $w_p$,
            \item $\share()$ of trace the empty word.
        \end{itemize}
        Given a sequence of action $s = act_1 act_2 \dots act_k$, we define the trace of $s$ by $\trace(s)$ the concatenation of the traces of the actions of $s$.
        
        % We denote $\duration(act)$ the function which associates to an action $act$ its corresponding duration.
        % Given a sequence of action $s = act_1 act_2 \dots act_k$, we define the duration of $s$ by $\duration(s) = \sum_{i=1}^k \duration(act_i)$, and the trace of $s$ by $\trace(s)$ the concatenation of the traces of the actions of $s$.
        % \Gabriel{trace est un mot, élément de $(\P \times \P)^*$}
        
\end{enumerate}

Note that hypotheses~\ref{comput-hyp:space} and~\ref{comput-hyp:time} are easily guaranteed since all awake robots are, transitively, awakened by robot $s$.
\Gabriel{Autre vision, suite à discussion avec Cyril: ce qui prend du temps c'est la distance à parcourir. Les noeuds peuvent compter ça à al volée, compter aussi les wait, et ça, on n'a qu'à dire que c'est $\time$}


\paragraph{Algorithm.}

A mono-execution is a tuple ($r, \exec)$ such that $r\in \R$ and $\exec$ is a sequence of actions $act_1, act_2, \dots$. % such that $act_i \in \{ \wait(t), \move(p,p'), \snap(p), \wakeup(r'), \share() \}$.

A mono-execution $(r, \exec)$ is space-valid if its trace $\trace(\exec) = \delta_1, \delta_2, \dots$ satisfies the following property: $\delta_i = w_p \Rightarrow \delta_{i-1} = m_p$.
Given two symbols $a\in\{m_p, w_p\}$ and $b\in \{m_{p'}, w_{p'}\}$, the duration of $(a,b)$, denoted $\duration(a,b)$ is defined as $|pp'|$.
The \emph{duration} of a space-valid mono-execution $(r, \exec)$, with trace $\delta_1, \delta_2, \dots$, denoted $\duration(r, \exec)$ is defined by:
\[
    \duration(w_{p_r}, \delta_1) + \sum_{i\geq1}\duration(\delta_i, \delta_{i+1}) + \sum_{\wait(t) \in \exec} t.
\]
%with $\delta_0 = w_{p_r}$.

~


    Given a mono-execution $(r,\exec)$, the \emph{trace} of $(r, \exec)$ is defined by moving index of action $act_i$, $\lmi(r, \exec, i)$ is:
    \[
        \lmi(r, \epsilon, i) =
        \left\{
            \begin{array}{ll}
                \max \{ j<i \mid act(j) = \move(p,p') \} & \text{if } \exists j<i: act(j) = \move(p,p') \\
                -1 & \text{otherwise} \\
            \end{array}
        \right.    
    \]positioning
    Given a mono-execution $(r,\epsilon)$, the starting position of action $act_i$, $\startp(r, \epsilon, i)$ is:
    \[
        \startp(r, \epsilon, i) =
        \left\{
            \begin{array}{ll}
                p' & \text{if } \lmi(r, \epsilon, i) \geq 0 \wedge  act_{\lmi(r, \epsilon, i)} = \move(p,p') \\
                p_r & \text{otherwise} \\
            \end{array}
        \right.    
    \]
    
    A mono-execution $(r, \epsilon)$ is space-valid if:
    
    \[
        \forall act_i \in \epsilon:
        \left\{
            \begin{array}{rlc}
                 act_i = \move(p, p') & \Rightarrow & p = \startp(r, \epsilon, i) \\
                 act_i = \snap(p) & \Rightarrow & p = \startp(r, \epsilon, i) \\
                 act_i = \wakeup(r') & \Rightarrow & p_{r'} = \startp(r, \epsilon, i) \\
            \end{array}
        \right.
    \]


A mono-execution $(r, \exec)$ is wake-valid if
\begin{itemize}
    \item $\wakeup(p, \underscore) \in \exec \Rightarrow p \neq p_r$
    \item $\wakeup(p, \underscore) \in \exec \Rightarrow \exists! act \in \exec: act = \wakeup(p, \underscore)$
\end{itemize}
We denote by $\children(r)$ the set of nodes $r'$ such that $\wakeup(p_{r'}, \underscore) \in \exec$.


A complete-execution $e$ is a map which associates to any robot $r$ of \R a sequence $\exec$ such that $(r, e(r))$ is a space-valid and wake-valid mono-execution, and such that the relation defined by $rRr' \iff r' \in \children(r)$ induces a tree rooted in $s$ with labels exactly $\R$. %, which we call Wake-up tree of the complete-execution $e$, and denote $\Tree(e)$.

Given a complete-execution and a robot $r\in\R\setminus\{s\}$, we denote by $\parent(r)$ the unique node $r'$ such that $r\in \children(r')$.
Given a complete-execution, we define
\Gabriel{Définir la temporalité des mono-executions, des robots, de la complete-execution.}
\Gabriel{J'ai oublié ce que je voulais dire ici...}

\Cyril{Remarque générale. Mettre un "." si c'est un \texttt{paragraph}, c'est à dire un titre sans retour de ligne, comme c'est le cas des définitions, théorèmes, etc. Pour les \texttt{section}, pas besoin en effet car y'a un saut de ligne. J'ai changé partout.}

\paragraph{Memory.}

Robots are given a set of variable, which are all initially empty, apart from the one which contains the (globally unique) identifier of the robot. Variables can be updated through the rules of the algorithm, or by two actions:

\begin{itemize}
    \item
        $\snap(p)$ returns the set of locations of the awake robots in $B_p(1)$, and of the sleeping robots in $B_p(1)$. \Gabriel{En fait il faudrait pouvoir distinguer les réveillés des endormis avec snap...}
    \item
        $\share()$ returns the set of states of the robots located at the same position than $r$ when executed.
\end{itemize}
